A modern approach to transition analysis and process mining with Markov models: A tutorial with R

This chapter presents an introduction to Markovian modeling for the analysis of sequence data. Contrary to the deterministic approach seen in the previous sequence analysis chapters, Markovian models are probabilistic models, focusing on the transitions between states instead of studying sequences as a whole. The chapter provides an introduction to this method and differentiates between its most common variations: first-order Markov models, hidden Markov models, mixture Markov models, and mixture hidden Markov models. In addition to a thorough explanation and contextualization within the existing literature, the chapter provides a step-by-step tutorial on how to implement each type of Markovian model using the R package seqHMM. The chaper also provides a complete guide to performing stochastic process mining with Markovian models as well as plotting, comparing and clustering different process models.

==> references.tex <==
@article{Rabiner1989,
	title        = {A Tutorial on Hidden {M}arkov Models and Selected Applications in Speech Recognition},
	author       = {Rabiner, Lawrence},
	year         = 1989,
	journal      = {Proceedings of the IEEE},
	publisher    = {IEEE},
	volume       = 77,
	number       = 2,
	pages        = {257--286},
	doi          = {10.1109/5.18626},
	owner        = {Satu Helske},
	timestamp    = {2014.04.14}
}
@misc{dynamitepaper,
	title        = {{dynamite}: an {R} Package for Dynamic Multivariate Panel Models},
	author       = {Santtu Tikka and Jouni Helske},
	year         = 2023,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.2302.01607},
	url          = {https://arxiv.org/abs/2302.01607}
}
@article{LMest,
	title        = {{LMest}: an {R} Package for Latent {M}arkov Models for Longitudinal Categorical Data},
	author       = {Francesco Bartolucci and Silvia Pandolfi and Fulvia Pennoni},
	year         = 2017,
	journal      = {Journal of Statistical Software},
	volume       = 81,
	number       = 4,
	pages        = {1--38},
	doi          = {10.18637/jss.v081.i04}
}
@manual{march,
	title        = {{march: Markov chains}},
	author       = {Ogier Maitre and Kevin Emery and with contributions from Oliver Buschor and Andre Berchtold},
	year         = 2020,
	url          = {https://CRAN.R-project.org/package=march},
	note         = {R package version 3.3.2}
}
@article{Berchtold,
	title        = {The double chain {M}arkov model},
	author       = {Andre Berchtold},
	year         = 1999,
	journal      = {Communications in Statistics - Theory and Methods},
	publisher    = {Taylor & Francis},
	volume       = 28,
	number       = 11,
	pages        = {2569--2589},
	doi          = {10.1080/03610929908832439},
	url          = {https://doi.org/10.1080/03610929908832439}
}
@article{Satu,
	title        = {The longitudinal association between engagement and achievement varies by time, students' profiles, and achievement state: a full program study},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles and Helske, Satu and Hrastinski, Stefan},
	year         = 2023,
	month        = jul,
	journal      = {Computers & Education},
	volume       = 199,
	pages        = 104787,
	abstract     = {There is a paucity of longitudinal studies in online learning across courses or throughout programs. Our study intends to add to this emerging body of research by analyzing the longitudinal trajectories of interaction between student engagement and achievement over a full four-year program. We use learning analytics and life-course methods to study how achievement and engagement are intertwined and how such relationship evolves over a full program for 106 students. Our findings have indicated that the association between engagement and achievement varies between students and progresses differently between such groups over time. Our results showed that online engagement at any single time-point is not a consistent indicator for high achievement. It takes more than a single point of time to reliably forecast high achievement throughout the program. Longitudinal high grades, or longitudinal high levels of engagement (either separately or combined) were indicators of a stable academic trajectory in which students remained engaged ---at least on average--- and had a higher level of achievement. On the other hand, disengagement at any time point was consistently associated with lower achievement among low-engaged students. Improving to a higher level of engagement was associated with ---at least--- acceptable achievement levels and rare dropouts. Lack of improvement or ``catching up'' may be a more ominous sign that should be proactively addressed.},
	keywords     = {Learning analytics; Multi-channel sequence analysis; Longitudinal engagement; Academic achievement; Mixture hidden Markov models; Student profiles; Person-centered methods}
}
@inproceedings{TEEM,
	title        = {From variables to states to trajectories ({VaSSTra)}: a method for modelling the longitudinal dynamics of learning and behaviour},
	author       = {L{\'o}pez-Pernas, Sonsoles and Saqr, Mohammed},
	year         = 2023,
	booktitle    = {Proceedings of the Tenth International Conference on Technological Ecosystems for Enhancing Multiculturality ({TEEM'22})},
	location     = {Salamanca, Spain},
	publisher    = {Springer},
	pages        = {in press},
	abstract     = {Research in learning analytics needs longitudinal studies that explore the learner's behaviour, disposition, and learning practices across time, a gap this article aims to bridge. We present VaSSTra: an innovative method for the longitudinal analysis of educational data that can be applied at different time scales (e.g., days, weeks, or courses), and allows the study of different aspects of learning as well as the factors that explain how such aspects evolve over time. Our method combines life- events methods with sequence analysis and consists of three steps: (1) converting variables to states (where variables are grouped into homogenous states); (2) from states to sequences (where the states are used to construct sequences across time), and (3) from sequences to trajectories (where similar sequences are grouped in trajectories). VaSSTra enables us to map the longitudinal unfolding of events while taking advantage of the wealth of life-events methods to visualize, model and describe the temporal dynamics of longitudinal activities. We demonstrate the method with a practical case study example.},
	conference   = {Technological Ecosystems for Enhancing Multiculturality (TEEM)}
}
@article{IHE,
	title        = {Intense, turbulent, or wallowing in the mire: a longitudinal study of cross-course online tactics, strategies, and trajectories},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles and Jovanovi{\'c}, Jelena and Ga{\v s}evi{\'c}, Dragan},
	year         = 2023,
	journal      = {The Internet and Higher Education},
	volume       = 57,
	pages        = 100902,
	abstract     = {Research has repeatedly demonstrated that students with effective learning strategies are more likely to have better academic achievement. Existing research has mostly focused on a single course or two, while longitudinal studies remain scarce. The present study examines the longitudinal sequence of students' strategies, their succession, consistency, temporal unfolding, and whether students tend to retain or adapt strategies between courses. We use a large dataset of online traces from 135 students who completed 10 successive courses (i.e., 1350 course enrollments) in a higher education program. The methods used in this study have shown the feasibility of using trace data recorded by learning management systems to unobtrusively trace and model the longitudinal learning strategies across a program. We identified three program-level strategy trajectories: a stable and intense trajectory related to deep learning where students used diverse strategies and scored the highest grades; a fluctuating interactive trajectory, where students focused on course requirements, scored average grades, and were relatively fluctuating; and a light trajectory related to surface learning where students invested the least effort, scored the lowest grades, and had a relatively stable pathway. Students who were intensely active were more likely to transfer the intense strategies and therefore, they were expected to require less support or guidance. Students focusing on course requirements were not as effective self-regulators as they seemed and possibly required early guidance and support from teachers. Students with consistent light strategies or low effort needed proactive guidance and support.},
	keywords     = {Learning analytics; Learning strategies; Sequence analysis; Longitudinal studies}
}
@article{Roles,
	title        = {How {CSCL} roles emerge, persist, transition, and evolve over time: a four-year longitudinal study},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles},
	year         = 2022,
	journal      = {Computers & Education},
	volume       = 189,
	pages        = 104581
}
@article{Bringing,
	title        = {Bringing synchrony and clarity to complex multi-channel data: A learning analytics study in programming education},
	author       = {L{\'o}pez-Pernas, Sonsoles and Saqr, Mohammed},
	year         = 2021,
	journal      = {IEEE Access},
	publisher    = {ieeexplore.ieee.org},
	volume       = 9,
	abstract     = {Supporting teaching and learning programming with learning analytics is an active area of inquiry. Most data used for learning analytics research comes from learning management …}
}
@article{Engagement,
	title        = {The longitudinal trajectories of online engagement over a full program},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles},
	year         = 2021,
	journal      = {Computers & Education},
	publisher    = {Elsevier},
	volume       = 175,
	pages        = 104325,
	abstract     = {Student engagement has a trajectory (a timeline) that unfolds over time and can be shaped by different factors including learners' motivation, school conditions, and the nature of …}
}
@incollection{ECTEL,
	title        = {The dire cost of early disengagement: a four-year learning analytics study over a full program},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles},
	year         = 2021,
	booktitle    = {{Technology-Enhanced} Learning for a Free, Safe, and Sustainable World},
	publisher    = {Springer International Publishing},
	address      = {Cham, Switzerland},
	series       = {Lecture Notes in Computer Science},
	pages        = {122--136}
}
@manual{BBmisc,
	title        = {{BBmisc}: Miscellaneous Helper Functions for {B. Bischl}},
	author       = {Bernd Bischl and Michel Lang and Jakob Bossek and Daniel Horn and Jakob Richter and Dirk Surmann},
	year         = 2022,
	url          = {https://CRAN.R-project.org/package=BBmisc},
	note         = {R package version 1.13}
}
@article{tidyLPA,
	title        = {{tidyLPA}: an {R} Package to Easily Carry Out Latent Profile Analysis ({LPA}) Using Open-Source or Commercial Software},
	author       = {Joshua M. Rosenberg and Patrick N. Beymer and Daniel J. Anderson and Caspar J. {Van Lissa} and Jennifer A. Schmidt},
	year         = 2018,
	journal      = {Journal of Open Source Software},
	volume       = 3,
	number       = 30,
	pages        = 978,
	doi          = {10.21105/joss.00978},
	url          = {https://joss.theoj.org/papers/10.21105/joss.00978}
}
@article{Gabadinho2011,
	title        = {Analyzing and Visualizing State Sequences in {R} with {TraMineR}},
	author       = {Alexis Gabadinho and Gilbert Ritschard and Nicolas S. Müller and Matthias Studer},
	year         = 2011,
	journal      = {Journal of Statistical Software},
	publisher    = {Foundation for Open Access Statistic},
	volume       = 40,
	number       = 4,
	doi          = {10.18637/jss.v040.i04},
	url          = {https://doi.org/10.18637/jss.v040.i04}
}
@manual{seqhandbook,
	title        = {{seqhandbook}: miscellaneous Tools for Sequence Analysis},
	author       = {Nicolas Robette},
	year         = 2023,
	url          = {https://CRAN.R-project.org/package=seqhandbook},
	note         = {R package version 0.1.1}
}
@article{Helske2019,
	title        = {Mixture Hidden {M}arkov Models for Sequence Data: The {seqHMM} Package in {R}},
	author       = {Satu Helske and Jouni Helske},
	year         = 2019,
	journal      = {Journal of Statistical Software},
	publisher    = {Foundation for Open Access Statistic},
	volume       = 88,
	number       = 3,
	doi          = {10.18637/jss.v088.i03},
	url          = {https://doi.org/10.18637/jss.v088.i03}
}
@manual{Gmisc,
	title        = {Gmisc: descriptive Statistics, Transition Plots, and More},
	author       = {Max Gordon},
	year         = 2023,
	url          = {https://CRAN.R-project.org/package=Gmisc},
	note         = {R package version 3.0.2}
}
@article{studer2013,
	title        = {{WeightedCluster} Library Manual: a practical guide to creating typologies of trajectories in the social sciences with {R}},
	author       = {Studer, Matthias},
	year         = 2013,
	journal      = {LIVES},
	doi          = {10.12682/LIVES.2296-1658.2013.24},
	url          = {https://www.centre-lives.ch/fr/bibcite/reference/84},
	date         = 2013
}
@article{Gabadinho2016,
	title        = {Analyzing State Sequences with Probabilistic Suffix Trees: the {PST} {R} Package},
	author       = {Alexis Gabadinho and Gilbert Ritschard},
	year         = 2016,
	journal      = {Journal of Statistical Software},
	volume       = 72,
	number       = 3,
	pages        = {1--39},
	doi          = {10.18637/jss.v072.i03}
}
@article{Liao2022,
	title        = {Sequence analysis: its past, present, and future},
	author       = {Tim F. Liao and Danilo Bolano and Christian Brzinsky-Fay and Benjamin Cornwell and Anette Eva Fasang and Satu Helske and Raffaella Piccarreta and Marcel Raab and Gilbert Ritschard and Emanuela Struffolino and Matthias Studer},
	year         = 2022,
	month        = sep,
	journal      = {Social Science Research},
	publisher    = {Elsevier {BV}},
	volume       = 107,
	pages        = 102772,
	doi          = {10.1016/j.ssresearch.2022.102772},
	url          = {https://doi.org/10.1016/j.ssresearch.2022.102772}
}
 
@incollection{LopezPernas2024,
	title        = {Modelling the Dynamics of Longitudinal Processes in Education. A tutorial with {R} for The {VaSSTra} Method},
	author       = {L{\'o}pez-Pernas, Sonsoles and Saqr, Mohammed},
	year         = 2024,
	booktitle    = {Learning analytics methods and tutorials: a practical guide using {R}},
	publisher    = {Springer},
	pages        = {in--press},
	editor       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles}
}
@article{vandePol1990,
	title        = {Mixed {M}arkov Latent Class Models},
	author       = {Frank van de Pol and Rolf Langeheine},
	year         = 1990,
	journal      = {Sociological Methodology},
	publisher    = {{JSTOR}},
	volume       = 20,
	pages        = 213,
	doi          = {10.2307/271087},
	url          = {https://doi.org/10.2307/271087}
}
@inbook{Vermunt,
	title        = {Latent class models in longitudinal research},
	author       = {J.K. Vermunt and B. Tran and J. Magidson},
	year         = 2008,
	booktitle    = {Handbook of Longitudinal Research},
	publisher    = {Elsevier},
	address      = {Netherlands},
	pages        = {373--385},
	isbn         = 9780123704818,
	note         = {Pagination: 696},
	language     = {English},
	editor       = {S. Menard}
}
@article{schwarz1978,
	title        = {Estimating the dimension of a model},
	author       = {Schwarz, Gideon E},
	year         = 1978,
	journal      = {The Annals of Statistics},
	publisher    = {The Institute of Mathematical Statistics},
	volume       = 6,
	number       = 2,
	pages        = {461--464},
	doi          = {10.1214/aos/1176344136}
}
@article{qgraph,
	title        = {{qgraph: network visualizations of relationships in psychometric data}},
	author       = {Sacha Epskamp and Ang\'{e}lique O. J. Cramer and Lourens J. Waldorp and Verena D. Schmittmann and Danny Borsboom},
	year         = 2012,
	journal      = {Journal of Statistical Software},
	volume       = 48,
	number       = 4
}
@manual{rio,
	title        = {{rio: a Swiss-army knife for data file I/O}},
	author       = {Chung-hong Chan and Geoffrey CH Chan and Thomas J. Leeper and Jason Becker},
	year         = 2021,
	note         = {R package version 0.5.29}
}
@manual{seqHMM,
	title        = {{seqHMM}: mixture hidden {Markov} models for social sequence data and other multivariate, multichannel categorical time series},
	author       = {Jouni Helske and Satu Helske},
	year         = 2023,
	url          = {https://cran.r-project.org/package=seqHMM},
	note         = {R package version 1.2.4}
}
@article{tidyverse,
	title        = {Welcome to the {tidyverse}},
	author       = {Hadley Wickham and Mara Averick and Jennifer Bryan and Winston Chang and Lucy D'Agostino McGowan and Romain François and Garrett Grolemund and Alex Hayes and Lionel Henry and Jim Hester and Max Kuhn and Thomas Lin Pedersen and Evan Miller and Stephan Milton Bache and Kirill Müller and Jeroen Ooms and David Robinson and Dana Paige Seidel and Vitalie Spinu and Kohske Takahashi and Davis Vaughan and Claus Wilke and Kara Woo and Hiroaki Yutani},
	year         = 2019,
	journal      = {Journal of Open Source Software},
	volume       = 4,
	number       = 43,
	pages        = 1686,
	doi          = {10.21105/joss.01686}
}
@techreport{latentgold,
	title        = {{Guide for Latent GOLD 5.1: Basic, Advanced, and Syntax}},
	author       = {J. K. Vermunt and J. Magidson},
	year         = 2016,
	address      = {Belmont, MA, U.S.A.},
	institution  = {Statistical Innovations Inc.}
}
@book{mplus,
	title        = {{Mplus User's Guide}},
	author       = {Muth\'{e}n, L. K. and Muth\'{e}n B. O.},
	year         = {1998--2017},
	publisher    = {Muth\'{e}n & Muth\'{e}n},
	address      = {Los Angeles, CA, U.S.A.},
	edition      = {Eighth edition}
}
@article{SAQR2022104581,
	title        = {How {CSCL} roles emerge, persist, transition, and evolve over time: a four-year longitudinal study},
	author       = {Mohammed Saqr and Sonsoles L{\'o}pez-Pernas},
	year         = 2022,
	journal      = {Computers & Education},
	volume       = 189,
	pages        = 104581,
	doi          = {https://doi.org/10.1016/j.compedu.2022.104581},
	issn         = {0360-1315},
	url          = {https://www.sciencedirect.com/science/article/pii/S036013152200152X}
}
@incollection{Lopez-Pernas2024-kf,
	title        = {Multi-channel sequence analysis in educational research: an introduction and tutorial with {R}},
	author       = {L{\'o}pez-Pernas, Sonsoles and Saqr, Mohammed and Murphy, Keefe},
	year         = 2024,
	booktitle    = {Learning analytics methods and tutorials: a practical guide using {R}},
	publisher    = {Springer},
	pages        = {in--press},
	editor       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles}
}
@incollection{Saqr2024-tv,
	title        = {Sequence analysis: Basic principles, technique, and tutorial},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles and Helske, Satu and Durand, Marion and Murphy, Keefe and Studer, Matthias and Ritschard, Gilbert},
	year         = 2024,
	booktitle    = {Learning analytics methods and tutorials: a practical guide using {R}},
	publisher    = {Springer},
	editor       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles}
}
@inbook{Helske2018,
	title        = {Combining Sequence Analysis and Hidden Markov Models in the Analysis of Complex Life Sequence Data},
	author       = {Helske, Satu and Helske, Jouni and Eerola, Mervi},
	year         = 2018,
	booktitle    = {Sequence Analysis and Related Approaches: Innovative Methods and Applications},
	publisher    = {Springer International Publishing},
	address      = {Cham},
	pages        = {185--200},
	doi          = {10.1007/978-3-319-95420-2_11},
	isbn         = {978-3-319-95420-2},
	editor       = {Ritschard, Gilbert and Studer, Matthias}
}
@misc{Muthen,
	title        = {Mplus: A General Latent Variable Modeling Program},
	author       = {Muth{\'e}n, Bengt and Muth{\'e}n, Linda},
	url          = {https://www.statmodel.com/download/Mplus-A%20General%20Latent%20Variable%20Modeling%20Program.pdf}
}
@article{Tormanen2022-ux,
	title        = {A person-centered approach to study students' socio-emotional interaction profiles and regulation of collaborative learning},
	author       = {{T{\"o}rm{\"a}nen} and {J{\"a}rvenoja} and {Saqr} and {Malmberg} and {others}},
	year         = 2022,
	journal      = {Frontiers in Education},
	issn         = {2504-284X}
}
@article{Tormanen2023-gz,
	title        = {Affective states and regulation of learning during socio-emotional interactions in secondary school collaborative groups},
	author       = {T{\"o}rm{\"a}nen, Tiina and J{\"a}rvenoja, Hanna and Saqr, Mohammed and Malmberg, Jonna and J{\"a}rvel{\"a}, Sanna},
	year         = 2023,
	month        = apr,
	journal      = {British Journal of Educational Psychology},
	publisher    = {Wiley},
	volume       = {93 Suppl 1},
	number       = {S1},
	pages        = {48--70},
	doi          = {10.1111/bjep.12525},
	issn         = {0007-0998, 2044-8279},
	language     = {en},
	pmid         = 35748024
}
@article{Fincham2019-yz,
	title        = {From Study Tactics to Learning Strategies: An Analytical Method for Extracting Interpretable Representations},
	author       = {Fincham, Ed and Ga{\v s}evi{\'c}, Dragan and Jovanovi{\'c}, Jelena and Pardo, Abelardo},
	year         = 2019,
	journal      = {IEEE Transactions on Learning Technologies.},
	volume       = 12,
	number       = 1,
	pages        = {59--72},
	doi          = {10.1109/TLT.2018.2823317},
	issn         = {1939-1382}
}
@inproceedings{Peeters2020-wa,
	title        = {Applying learning analytics to map students' self-regulated learning tactics in an academic writing course},
	author       = {Peeters, Ward and Saqr, Mohammed and Viberg, Olga},
	year         = 2020,
	booktitle    = {Proceedings of the 28th International Conference on Computers in Education},
	volume       = 1,
	pages        = {245--254}
}
@article{Lim2023-kg,
	title        = {Effects of real-time analytics-based personalized scaffolds on students' self-regulated learning},
	author       = {Lim, Lyn and Bannert, Maria and van der Graaf, Joep and Singh, Shaveen and Fan, Yizhou and Surendrannair, Surya and Rakovic, Mladen and Molenaar, Inge and Moore, Johanna and Ga{\v s}evi{\'c}, Dragan},
	year         = 2023,
	month        = feb,
	journal      = {Computers in Human Behavior},
	publisher    = {Elsevier BV},
	volume       = 139,
	number       = 107547,
	pages        = 107547,
	doi          = {10.1016/j.chb.2022.107547},
	issn         = {0747-5632, 1873-7692},
	url          = {https://www.sciencedirect.com/science/article/pii/S0747563222003673},
	copyright    = {http://creativecommons.org/licenses/by/4.0/},
	keywords     = {Self-regulated learning; Learning analytics; Personalized scaffolds; Adaptive support; Process mining; Trace data},
	language     = {en}
}
@article{Saqr2023-he,
	title        = {The temporal dynamics of online problem-based learning: Why and when sequence matters},
	author       = {Saqr, Mohammed and L{\'o}pez-Pernas, Sonsoles},
	year         = 2023,
	month        = mar,
	journal      = {International Journal of Computer-Supported Collaborative Learning},
	volume       = 18,
	number       = 1,
	pages        = {11--37},
	doi          = {10.1007/s11412-023-09385-1},
	issn         = {1556-1615},
	url          = {https://doi.org/10.1007/s11412-023-09385-1}
}
@article{BOUGUETTAYA20152785,
	title        = {Efficient agglomerative hierarchical clustering},
	author       = {Athman Bouguettaya and Qi Yu and Xumin Liu and Xiangmin Zhou and Andy Song},
	year         = 2015,
	journal      = {Expert Systems with Applications},
	volume       = 42,
	number       = 5,
	pages        = {2785--2797},
	doi          = {https://doi.org/10.1016/j.eswa.2014.09.054},
	issn         = {0957-4174},
	keywords     = {Clustering analysis, Hybrid clustering, Data mining, Data distribution, Coefficient of correlation}
}
@inproceedings{Gilpin13,
	title        = {Efficient Hierarchical Clustering of Large High Dimensional Datasets},
	author       = {Gilpin, Sean and Qian, Buyue and Davidson, Ian},
	year         = 2013,
	booktitle    = {Proceedings of the 22nd ACM International Conference on Information \& Knowledge Management},
	location     = {San Francisco, California, USA},
	publisher    = {Association for Computing Machinery},
	address      = {New York, NY, USA},
	series       = {CIKM '13},
	pages        = {1371–1380},
	doi          = {10.1145/2505515.2505527},
	isbn         = 9781450322638,
	url          = {https://doi.org/10.1145/2505515.2505527},
	numpages     = 10,
	keywords     = {hierarchical clustering, binary codes}
}
@article{Matcha2020-jp,
	title        = {Analytics of Learning Strategies: Role of Course Design and Delivery Modality},
	author       = {Matcha, Wannisa and Ga{\v s}evi{\'c}, Dragan and Ahmad Uzir, Nora'ayu and Jovanovi{\'c}, Jelena and Pardo, Abelardo and Lim, Lisa and Maldonado-Mahauad, Jorge and Gentili, Sheridan and P{\'e}rez-Sanagust{\'\i}n, Mar and Tsai, Yi-Shan},
	year         = 2020,
	journal      = {Journal of Learning Analytics},
	publisher    = {SoLAR},
	volume       = 7,
	number       = 2,
	pages        = {45--71},
	doi          = {10.18608/jla.2020.72.3},
	issn         = {1929-7750}
}
@article{Boroujeni2019-vf,
	title        = {Discovery and Temporal Analysis of {MOOC} Study Patterns},
	author       = {Boroujeni, Mina Shirvani and Dillenbourg, Pierre},
	year         = 2019,
	journal      = {Journal of Learning Analytics},
	publisher    = {SoLAR},
	volume       = 6,
	number       = 1,
	pages        = {16--33},
	doi          = {10.18608/jla.2019.61.2},
	issn         = {1929-7750, 1929-7750}
}
@article{Kokoc2021-rc,
	title        = {Unfolding Students' Online Assignment Submission Behavioral Patterns using Temporal Learning Analytics},
	author       = {Koko{\c c}, Mehmet and Ak{\c c}ap{\i}nar, G{\"o}khan and Hasnine, Mohammad Nehal},
	year         = 2021,
	journal      = {Educational Technology \& Society},
	publisher    = {International Forum of Educational Technology \& Society},
	volume       = 24,
	number       = 1,
	pages        = {223--235},
	issn         = {1436-4522},
	url          = {https://www.jstor.org/stable/26977869}
}
@article{Andrade2017-we,
	title        = {A Measurement Model of Gestures in an Embodied Learning Environment: Accounting for Temporal Dependencies},
	author       = {Andrade, Alejandro and Danish, Joshua A and Maltese, Adam V},
	year         = 2017,
	journal      = {Journal of Learning Analytics},
	publisher    = {SoLAR},
	volume       = 4,
	number       = 3,
	pages        = {18--46},
	doi          = {10.18608/jla.2017.43.3},
	issn         = {1929-7750, 1929-7750},
	url          = {https://www.learning-analytics.info/index.php/JLA/article/view/5418},
	language     = {en}
}

@inproceedings{Gatta2017-rg,
	title        = {Generating and comparing knowledge graphs of medical processes using {pMineR}},
	author       = {Gatta, Roberto and Vallati, Mauro and Lenkowicz, Jacopo and Rojas, Eric and Damiani, Andrea and Sacchi, Lucia and De Bari, Berardino and Dagliati, Arianna and Fernandez-Llatas, Carlos and Montesi, Matteo and Marchetti, Antonio and Castellano, Maurizio and Valentini, Vincenzo},
	year         = 2017,
	booktitle    = {Proceedings of the Knowledge Capture Conference},
	location     = {Austin TX USA},
	publisher    = {ACM},
	address      = {New York, NY, USA},
	doi          = {10.1145/3148011.3154464},
	isbn         = 9781450355537,
	url          = {http://dx.doi.org/10.1145/3148011.3154464},
	copyright    = {http://www.acm.org/publications/policies/copyright\_policy\#Background},
	conference   = {K-CAP 2017: Knowledge Capture Conference}
}

@article{Helske2023,
  title={Predicting the stability of early employment with its timing and childhood social and health-related predictors: a mixture Markov model approach},
  author={Helske, Satu and Keski-S{\"a}ntti, Markus and Kivel{\"a}, Juha and Juutinen, Aapo and K{\"a}{\"a}ri{\"a}l{\"a}, Antti and Gissler, Mika and Merikukka, Marko and Lallukka, Tea},
  journal={Longitudinal and Life Course Studies},
  volume={14},
  number={1},
  pages={73--104},
  year={2023},
  publisher={Bristol University Press}
}

==> title.tex <==
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$

$if(subtitle)$
\subtitle{$subtitle$}
$endif$

$for(by-author)$
\author$if(it.metadata.affil-id)$[$it.metadata.affil-id$]$endif${$it.name.literal$}
$endfor$

$if(by-affiliation)$
$for(by-affiliation)$
\affil[$it.id$]{$it.name$}
$endfor$
$endif$


\date{$date$}
